Convergence and Stability of Coupled Belief--Strategy Learning Dynamics in Continuous Games

We propose a learning dynamics to model how strategic agents repeatedly play a continuous game while relying on an information platform to learn an unknown payoff-relevant parameter. In each time step, the platform updates a belief estimate of the parameter based on players' strategies and realized payoffs using Bayes's rule. Then, players adopt a generic learning rule to adjust their strategies based on the updated belief. We present results on the convergence of beliefs and strategies and the properties of convergent fixed points of the dynamics. We obtain sufficient and necessary conditions for the existence of globally stable fixed points. We also provide sufficient conditions for the local stability of fixed points. These results provide an approach to analyzing the long-term outcomes that arise from the interplay between Bayesian belief learning and strategy learning in games, and enable us to characterize conditions under which learning leads to a complete information equilibrium.

==> proof_applications.tex <==
%%novalidate
% !TEX root = main041620.tex
\noindent\textbf{\emph{Proof of Proposition \ref{prop:complete}.}} 

\vspace{0.2cm}
\noindent\textbf{\emph{Proof of Proposition \ref{prop:map_convergence}}
.} 
First, since the Bayesian belief $\thetat$ given by \eqref{eq:update_belief} converges to a fixed point belief $\thetabar$ and $\thetat_M = \argmax_{\s \in \S} \thetat(\s)$, we know that $\lim_{\t \to \infty} \thetat_M= \thetabar_M$, where $\thetabar_M = \argmax_{\s \in \S} \thetabar(\s)$ with probability 1. Second, analogous to Lemma \ref{lemma:q_eq}, we can show that $\lim_{\t \to \infty} \qt= \qbar=\gwe(\thetabar_M)$ in learning with equilibrium strategies under \textbf{(A1)} -- \textbf{(A2)}. Additionally, we know from Lemma \ref{lemma:consistency} that $\lim_{\t \to \infty}\thetat(\s) = 0$ for $\s \in \S \setminus \Sequiv(\qbar)$. Therefore, $\thetabar_M = \argmax_{\s \in \S} \thetabar(\s)$ must be in the set $\Sequiv(\qbar)$. Finally, analogous to Lemma \ref{lemma:q_br}, we can show that $\lim_{\t \to \infty} d\(\qt, \EQ(\thetabar_M)\)=0$ in learning with best response strategies under \textbf{(A3)} -- \textbf{(A6)}. Additionally, we know from the proof of Lemma \ref{lemma:constrained_set} that $\lim_{\t \to \infty}\thetat(\s) = 0$ for $\s \in \S \setminus \Sequiv(\Qbar)$, where $\Qbar$ is the limit set of sequence $\(\qt\)_{\t=1}^{\infty}$. Therefore, $\thetabar_M = \argmax_{\s \in \S} \thetabar(\s)$ must be in the set $\Sequiv(\Qbar)$. 
\QEDA




